The Unbalanced Gromov Wasserstein Distance: Conic Formulation and Relaxation

Comparing metric measure spaces (i.e. a metric space endowed with aprobability distribution) is at the heart of many machine learning problems. The most popular distance between such metric measure spaces is theGromov-Wasserstein (GW) distance, which is the solution of a quadratic assignment problem. The GW distance is however limited to the comparison of metric measure spaces endowed with a probability distribution. To alleviate this issue, we introduce two Unbalanced Gromov-Wasserstein formulations: a distance and a more tractable upper-bounding relaxation.They both allow the comparison of metric spaces equipped with arbitrary positive measures up to isometries. The first formulation is a positive and definite divergence based on a relaxation of the mass conservation constraint using a novel type of quadratically-homogeneous divergence. This divergence works hand in hand with the entropic regularization approach which is popular to solve large scale optimal transport problems. We show that the underlying non-convex optimization problem can be efficiently tackled using a highly parallelizable and GPU-friendly iterative scheme. The second formulation is a distance between mm-spaces up to isometries based on a conic lifting. Lastly, we provide numerical experiments onsynthetic examples and domain adaptation data with a Positive-Unlabeled learning task to highlight the salient features of the unbalanced divergence and its potential applications in ML.

==> sections/2-background_uot_v1.tex <==
\section{Background on the conic formulation of UOT}
\label{sec-background}

Following~\cite{liero2015optimal}, this section reviews and generalizes the derivation of the conic formulation from UW~\eqref{eq-uw}. A detailed version of this construction is presented in Appendix~\ref{sec-app-background}.
%
Our relaxed divergence UGW and conic distance CGW defined in Section~\ref{sec-distance} build upon those constructions but are not anymore equal due to the non-convexity of GW problems.

The starting point is to reformulate UW~\eqref{eq-uw} by decomposing the Csiszar divergences. It reads
\begin{equation}
\begin{aligned}\label{eq-uw-reverse}
\text{UW}(\mu,\nu)^q = \uinf{\pi \in \Mm(X^2)} &\int L_{\C(d(x,y))}(\f(x), \g(y))\d\pi(x,y)
+\psi^\prime_\infty(|\mu^\bot| + |\nu^\bot|),
\end{aligned}
\end{equation}
where $L_{c}(r,s) \eqdef c + r\phi(1/r) + s\phi(1/s)$, with $|\mu^\bot|\eqdef\mu^\bot(X)$ and $(\f \eqdef \frac{\d\mu}{\d\pi_1}, \g \eqdef \frac{\d\nu}{\d\pi_2})$ are the densities of the Lebesgue decomposition of $(\mu,\nu)$ with respect to $(\pi_1,\pi_2)$ that read
$\mu = \f \pi_1 + \mu^\bot$ and $\nu = \g \pi_2 + \nu^\bot$.
The term $(|\mu^\bot| + |\nu^\bot|)$ penalize pure mass creation/destruction and $L_{\C(d)}$ can be interpreted as a new transport cost.

Then the authors of~\cite{liero2015optimal} define the 1-homogeneous function $H_c \eqdef \inf_{\theta\geq 0} \theta L_c(\tfrac{r}{\theta}, \tfrac{s}{\theta})$ as the perspective transform of $L_c$
%\begin{align}\label{eq-def-homog-persp}
%	H_c(r, s) \eqdef \inf_{\theta\geq 0} \theta\big( c + \psi(\tfrac{r}{\theta}) + \psi(\tfrac{s}{\theta} ) \big) 
%	= \inf_{\theta\geq 0} \theta L_c(\tfrac{r}{\theta}, \tfrac{s}{\theta}).
%\end{align}
By definition one has $L_c\geq H_c$. Such idea stems from the optimization of $\pi(x,y)$ with a pointwise scaling $\theta$. Then spaces variables $x$ are lifted as $(x,r)$, where $r$ accounts for the mass at $x$. Since $H_c$ is homogeneous in $(r,s)$, variables are represented in the cone set $\Co[X] = X\times\RR_+ / (X\times\{0\})$, where
coordinates of the form $(x,0)$ are merged into a single point called the apex of the cone, noted $\zc_X$. In the sequel, points of $X\times\RR_+$ are noted $(x,r)$ and those of $\Co[X]$ are noted $[x,r]$ to emphasize the quotient operation at the apex.
For a pair $(p,q)\in\RR_+$, we define a cost for any $[x,r],[y,s]\in\Co[X]^2$ as $\Dd_{\Co[X]}([x,r], [y,s])^q \eqdef H_{\C(d(x,y))}(r^p, s^p)$.
In general $\Dd_{\Co[X]}$ is not a distance, but it is always definite as stated by this result proved in Appendix~\ref{sec-app-background}.
\begin{proposition}\label{prop-cone-dist-definite}
	Assume that $d$ is definite, $\C^{-1}(\{0\})=\{0\}$ and $\phi^{-1}(\{0\})=\{1\}$. Assume also that for any $(r,s)$, there always exists $\theta^*$ such that $H_c(r, s)= \theta^* L_c(\tfrac{r}{\theta^*}, \tfrac{s}{\theta^*})$.
	Then $\Dd_{\Co[X]}$ is definite on $\Co[X]$, i.e. $\Dd_{\Co[X]}([x,r], [y,s]) =0$ if and only if $(r=s=0) \;\textrm{or}\; (r=s \;\textrm{and}\; x=y)$.
\end{proposition}
%\begin{proof}
%	Assume $\Dd_{\Co[X]}([x,r], [y,s]) =0$, and write $\theta^*$ such that
%	\begin{align*}
%		\Dd_{\Co[X]}([x,r], [y,s])^q = \theta^* L_c(\tfrac{r^p}{\theta^*}, \tfrac{s^p}{\theta^*})
%		= \theta^* \C(d(x,y)) + r^p\phi(\tfrac{\theta^*}{r^p}) + s^p\phi(\tfrac{\theta^*}{s^p}).
%	\end{align*}
%	There are two cases. If $\theta^* >0$, since all terms are positive, they are all equal to $0$. By definiteness of $d$ it yields $x=y$ and because $\phi^{-1}(\{0\})=\{1\}$ we have $r^p=s^p=\theta^*$ and $r=s$.
%	If $\theta^*=0$ then $\Dd_{\Co[X]}([x,r], [y,s])^q=\phi(0)(r^p+s^p)$. The assumption $\phi^{-1}(\{0\})=\{1\}$ implies $\phi(0)>0$, thus necessarily $r=s=0$.
%\end{proof} 
The function $H_c$ can be computed in closed form for a certain number of common entropies $\phi$, and we refer to~\cite[Section 5]{liero2015optimal} for an overview. 
%
Of particular interest are those $\phi$ where $\Dd_{\Co[X]}$ is a distance, which necessitates a careful choice of $\C,p$ and $q$. We now detail three particular settings where this is the case. In each setting we provide $(\D_\phi, \C, p, q)$ and its associated cone distance $\Dd_{\Co[X]}$. 
\paragraph{Gaussian Hellinger distance (GH).} One takes $\D_\phi = \KL$, $\C(t) = t^2$, $q=p=2$ and
\begin{align*}
	\Dd_{\Co[X]}([x,r], [y,s])^2 = r^2 + s^2 - 2rse^{-d(x,y) / 2}.
\end{align*}
\paragraph{Hellinger-Kantorovich (HK) / Wasserstein-Fisher-Rao distance (WFR).} It corresponds to $\D_\phi =\KL$, $\C(t) = -\log\cos^2(t\wedge\tfrac{\pi}{2})$, $q=p=2$ and
\begin{align*}
	\Dd_{\Co[X]}([x,r], [y,s])^2 = r^2 +s^2 - 2rs\cos(\tfrac{\pi}{2}\wedge d(x,y)).
\end{align*}
\paragraph{Partial optimal transport (PT).}	One takes $\D_\phi = \TV$, $\C(t)=t^q$, $q\geq 1$, $p=1$ and
\begin{align*}
	\Dd_{\Co[X]}([x,r], [y,s])^q = r + s - (r\wedge s)(2-d(x,y)^q)_+.
\end{align*}
It is proved in~\citet{liero2015optimal, burago2001course, chizat2018unbalanced} that $\Dd_{\Co[X]}$ is a cone distance. The setting of HK/WFR might seem peculiar, but it makes unbalanced OT a length space induced by the GH distance when $d$ is a geodesic distance on $X$. PT and HK/WFR introduce cut-offs, i.e. there is no transport between points too far from each other, e.g. in the latter case $\C(d(x,y))=+\infty$ if $d(x,y)>\pi/2$. The cut-off can be modified by scaling $\la \mapsto \la(\cdot/s)$ for some cutoff $s$.

The conic formulation~\eqref{eq-uw-conic} consists in solving an OT problem on the cone, with the addition of two linear constraints. Informally speaking, $H_c$ becomes $\Dd_{\Co[X]}$, the term $(|\mu^\bot| + |\nu^\bot|)$ is taken into account by the constraints~\eqref{eq-uw-conic-set} below, and the variables $(\f,\g)$ are replaced by $(r^p,s^p)$. It reads
\begin{align}\label{eq-uw-conic}
	\text{CUW}(\mu,\nu)^q \eqdef \inf_{\al\in \Uu_p(\mu,\nu)} \int \Dd_{\Co[X]}([x, r], [y, s]))^q\d\al([x,r], [y,s]),
\end{align}
where the constraint set $\Uu_{p}(\mu,\nu)$ is defined as
\begin{align}\label{eq-uw-conic-set}
	\Uu_{p}(\mu,\nu)  \eqdef \enscond{ \al\in\Mm_+(\Co[X]^2) }{
		\int_{\RR_+} r^p \d\al_1(\cdot,r)=\mu,
		\int_{\RR_+} s^p \d\al_2(\cdot,s)=\nu
	}.
\end{align}
Thus CUW consists in minimizing the Wasserstein distance $\text{W}_{\Dd_{\Co[X]}}(\al_1,\al_2)$ on the cone $(\Co[X], \Dd_{\Co[X]})$. The additional constraints on $(\al_1,\al_2)$ means that the lift on the cone must be consistent with the input $(\mu,\nu)$. When $\Dd_{\Co[X]}$ is a distance, CUW inherits the metric properties of $W_{\Dd_{\Co[X]}}$. Our theoretical results rely on an analog construction for GW.


The following proposition states the equality of the three formulations and recapitulates its main properties. The proofs are detailed in~\cite{liero2015optimal}.
\begin{proposition}[From~\cite{liero2015optimal}]
	One has $\text{\upshape{UW}}=\text{\upshape{CUW}}$, which are symmetric, positive and definite.
	Furthermore, if $(X,d_X)$ and $(\Co[X], \Dd_{\Co[X]})$ are metric spaces with $X$ separable, then $\Mm_+(X)$ endowed with $\text{\upshape{CUW}}$ is a metric space.
\end{proposition}
%\begin{proof}
%	The equality $\text{UW}=\text{HUW}$ is given by~\cite[Theorem 5.8]{liero2015optimal}, while the equality $\text{HUW}=\text{CUW}$ holds thanks to~\cite[Theorem 6.7 and Remark 7.5]{liero2015optimal}, where the latter theorem can be straightforwardly generalized to any cone distance defined by~\eqref{eq-def-cone-dist}. Since $\Dd_{\Co[X]}$ is symmetric, positive and definite (see Proposition~\ref{prop-cone-dist-definite}), then so is CUW. Furthermore, if $\Dd_{\Co[X]}$ satisfies the triangle inequality, separability of $X$ allows to apply the gluing lemma~\cite[Corollary 7.14]{liero2015optimal} which generalizes to any exponent $p$ defining $\Uu_{p}(\mu,\nu)$ and any cone distance $\Dd_{\Co[X]}$.
%\end{proof}


==> sections/3-ugw_distance_v2.tex <==
% !TEX root = ../iclr2021_submission.tex

\section{Unbalanced Gromov-Wasserstein formulations}
\label{sec-distance}

We present in this section our two new formulations and their properties. The first one, called UGW, is exploited in Sections~\ref{sec-algo} and~\ref{sec-xp} to derive an efficient algorithm used in numerical experiments. The second one, called CGW, defines a distance between mm-spaces up to isometries. Those results build upon the results of~\citet{liero2015optimal}, and a summary of the construction of UOT is detailed in Appendix~\ref{sec-app-background}.
%
In all what follows, we consider complete separable mm-spaces endowed with a metric and a positive measure.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The unbalanced Gromov-Wasserstein divergence}

This new formulation makes use of quadratic $\phi$-divergences, defined as $\D_\phi^\otimes(\rho|\nu) \eqdef \D_\phi(\rho \otimes \rho|\nu \otimes \nu)$, where $\rho \otimes \rho \in \Mm_+(X^2)$ is the tensor product measure defined by $\d(\rho \otimes \rho)(x,y)=\d\rho(x)\d\rho(y)$.
%
Note that $\D_\phi^\otimes$ is not a convex function in general.

\begin{definition}[Unbalanced GW]
The Unbalanced Gromov-Wasserstein divergence is defined as $\UGW(\Xx, \Yy) = \inf_{\pi\in\Mmp(X\times Y)} \Ll(\pi)$ where
\begin{equation}\label{eq-ugw-func}
\begin{aligned}
  \Ll(\pi) \eqdef \Gg(\pi)
   + \D_\phi^\otimes(\pi_1|\mu) + \D_\phi^\otimes(\pi_2|\nu).
\end{aligned}
\end{equation}
\end{definition}

This definition can be understood as an hybridation between~\eqref{eq-uw} and~\eqref{eq-defn-gw} but with a twist: one needs to use the quadratic divergence $\D_\phi^\otimes$ in place of $\D_\phi$. To the best of our knowledge, it is the first time such quadratic divergences are being used and studied.
%
In the TV case, this is the most important distinction between UGW and partial GW~\citep{chapel2020partial}.
%
%
Note also that the balanced GW distance~\eqref{eq-defn-gw}  is recovered as a particular case when using $\phi=\iota_{\{1\}}$ or by letting $\rho \rightarrow +\infty$ for an entropy $\psi=\rho\phi$.

Using quadratic divergences results in UGW being 2-homogeneous: 
%\redrm{if $\mu$ and $\nu$ are multiplied by $\th \geq 0$, then $\UGW(\Xx, \Yy)$ is multiplied by $\th^2$.} 
%
for $\th\geq 0$, writing $(\Xx_\th, \Yy_\th)$ equiped with $(\th\mu,\th\nu)$, one has $\th^{-2}\UGW(\Xx_\th, \Yy_\th)=\UGW(\Xx, \Yy)$.
%
%\blue{Using $\D_\phi$ instead of $\D_\phi^\otimes$ makes the problem degenerate: writing $\tilde{\UGW}$ the problem penalized with $\D_\phi$, one has $\lim_{\th\rightarrow\infty} \th^{-2}\tilde{\UGW}(\Xx_\th, \Yy_\th)=0$ and $\lim_{\th\rightarrow\infty} \th^{-1}\tilde{\UGW}(\Xx_\th, \Yy_\th)=+\infty$}.
%
When using non tensorized $\phi$-divergences, the resulting unbalanced Gromov-Wassertein functional between $\Xx_\th$ and $\Yy_\th$ have very different and inconsistent behaviors when $\theta\rightarrow 0$ and $\theta\rightarrow +\infty$. Indeed, once normalized by $\th^{-2}$ and $\th^{-1}$, one obtains respectively balanced GW and a Hellinger-type distance. Using tensorized divergences ensure that the behavior does not depends on $\th$.
%
%\redrm{Not using such divergences results in a lack of} \blue{The} 2-homogeneity of $\Ll$ is crucial to show the connection between our proposed formulations.


We first prove the existence of optimal plans $\pi$ solution to~\eqref{eq-ugw-func}, which holds for the three key settings of Section~\ref{sec-setup-dist}, namely for $\KL$, $\TV$, and for compact metric spaces (such as finite pointclouds and graphs). All proofs are deferred in Appendix~\ref{appendix-distance-ugw}.
\begin{proposition}[Existence of minimizers]\label{thm-exist-minimizer}
	We assume that $(X,Y)$ are compact and that either (i) $\phi$ superlinear, i.e $\phi^\prime_\infty=\infty$, or (ii) $\C$ has compact sublevel sets in $\RR_+$ and $2\phi^\prime_\infty + \inf \C >0$.
	Then there exists $\pi\in\Mm_+(X\times Y)$ such that $\UGW(\Xx,\Yy)=\Ll(\pi)$.
\end{proposition}
The following proposition ensures that the functional $\UGW$ can be used to compare mm-spaces.
\begin{proposition}[Definiteness of UGW]\label{prop-ugw-definite}
Assume that $\phi^{-1}(\{0\})=\{1\}$ and $\C^{-1}(\{0\})=\{0\}$. Then $\UGW(\Xx,\Yy) \geq 0$ and is $0$ if and only if $\Xx\sim\Yy$.
\end{proposition}
%\begin{proof}
%	Assume $\UGW(\Xx,\Yy)=0$. Positivity implies that all the terms appearing in $\Ll$ are zero. Similarly to the balanced case~\cite{memoli2011gromov}, the distortion being zero imposes that the plan $\pi$ defines an isometry. The $\phi$-divergences being zero implies that $\pi$ has marginals equal to $(\mu,\nu)$. This plan thus defines an isometric bijection between $\Xx$ and $\Yy$, see Appendix~\ref{appendix-distance-ugw} for details.
%\end{proof}

We end this section with a reformulation of UGW~\eqref{eq-ugw-func} which is important to make the connection with the second formulation of the following section. Its proof is deferred to Appendix~\ref{appendix-distance-ugw}. 
%
It splits UGW into two parts: the term $\phi(0)(|(\mu\otimes\mu)^\bot| + |(\nu\otimes\nu)^\bot|)$  accounts for the pure creation/destruction of mass and a new transport cost $L_c$ accounts for the remaining part (partial/pure transport and partial creation/destruction of mass).

\begin{lemma}\label{lem-rewrite-ugw}
	Defining $L_{c}(a,b) \eqdef c + a\phi(1/a) + b\phi(1/b)$, and writing $(\f \eqdef \frac{\d\mu}{\d\pi_1}, \g \eqdef \frac{\d\nu}{\d\pi_2})$ the Lebesgue densities of $(\mu,\nu)$ w.r.t. $(\pi_1,\pi_2)$ such that
	$\mu = \f \pi_1 + \mu^\bot$ and $\nu = \g \pi_2 + \nu^\bot$, one has
	\begin{equation}
		\begin{aligned}\label{eq-rewrite-ugw}
		\Ll(\pi)= &\int_{X^2 \times Y^2} L_{\C(|d_X - d_Y|)}(\f\otimes\f,\g\otimes\g)\d\pi\d\pi +\phi(0)(|(\mu\otimes\mu)^\bot| + |(\nu\otimes\nu)^\bot|).
		\end{aligned}
	\end{equation}
\end{lemma}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The conic Gromov-Wasserstein distance}

We introduce a second ``conic'' formulation of unbalanced GW, which is connected to UGW, and whose construction is inspired by the conic formulation of UOT (see Appendix~\ref{sec-app-background} for an overview). % The main contribution is Theorem~\ref{thm-ugw-dist} which states that it defines a distance between mm-spaces equipped with arbitrary positive measures.


\subsubsection{Background on cone sets and distances}
\label{sec-setup-dist}

The conic formulation lifts a point $x \in X$ to a couple $(x,r) \in X \times \RR^+$ where $r$ encodes some (power of a) mass.
%
Then we seek optimal transport plans defined over $\Co[X] \eqdef X\times\RR_+ / (X\times\{0\})$, where coordinates $(x,r=0)$ with no mass are merged into a single point $\zc_{X}$ called the apex of the cone. In the sequel, points of $X\times\RR_+$ are noted $(x,r)$, while $[x,r]$ are quotiented points of $\Co[X]$. %are noted .


While transport plans depend on variables  $([x,r],[y,s])$ and $([x',r'],[y',s'])$ in $\Co[X]\times\Co[Y]$, the transportation cost involved in our conic formulation only makes use of the 2-D cone $\Co[\RR_+]$ over $\RR_+$ endowed with the distance $|u-v|$ (note that any other distance on $\RR$ could be used as well).
%
More specifically, we consider coordinates of the form $([u,a],[v,b]) = ([d_X(x,x'),rr'], [d_Y(y,y'),ss']) \in \Co[\RR_+] \times \Co[\RR_+]$.
%
Thus we now describe conic discrepancies $\Dd$ on $\Co[\RR_+]$, which are defined for $(p,q) \geq 0$ as
\begin{equation}
	\begin{aligned}
	\Dd([u,a], [v,b])^q \eqdef H_{\C(|u-v|)}(a^p, b^p)\,,
	\qwhereq
	H_c(a^p, b^p) \eqdef \inf_{\theta\geq 0} \theta L_c(\tfrac{a^p}{\theta}, \tfrac{b^p}{\theta})\,,
	\end{aligned}
\end{equation}

	

is the perspective transform of $L_c$ introduced in Lemma~\ref{lem-rewrite-ugw}.
%
The intuition underpinning the definition of this cost is that the perspective transform accounts for the possibility to rescale a transport plan $\pi$ by a scalar $\th$ 
%\redrm{at each points in the cone} 
but the scaling is performed pointwise instead of globally.
%
In general $\Dd$ is not a distance, but it is always definite as stated by this result proved in Appendix~\ref{sec-app-background}.

\begin{proposition}\label{prop-cone-dist-definite}
	Assume $\C^{-1}(\{0\})=\{0\}$, $\phi^{-1}(\{0\})=\{1\}$ and $\phi$ is coercive. 
	%Assume also that for any $(a,b)$, there always exists $\theta$ such that $H_c(a,b)= \theta L_c(\tfrac{a}{\theta}, \tfrac{b}{\theta})$.
	Then $\Dd$ is definite on $\Co[\RR^+]$, i.e. $\Dd([u,a], [v,b]) =0$ if and only if $(a=b=0) \;\textrm{or}\; (a=b \;\textrm{and}\; u=v)$.
\end{proposition}
% The function $H_c$ can be computed in closed form for a certain number of common entropies $\phi$, and we refer to~\citet[Section 5]{liero2015optimal} for an overview.
%
Of particular interest are those $\phi$ where $\Dd$ is a distance, which necessitates a careful choice of $\C,p$ and $q$.
We now detail three examples where this is the case.
% In each setting we provide $(\D_\phi, \C, p, q)$ and its associated cone distance $\Dd$. We focus here on the Euclidean distance, but it generalizes to any metric $d(u,v)$.
\vspace*{-0.35cm}
\paragraph{Gaussian Hellinger distance (GH).}
When $\D_\phi = \KL$, $\C(t) = t^2$ and $q=p=2$, then one has
%\begin{align*}
	$\Dd([u,a], [v,b])^2 = a^2 + b^2 - 2abe^{-|u-v| / 2}$. This cone distance~\citep{burago2001course} is further generalized by~\cite{de2019metric} who shows that $\Dd$ is a distance for power entropies $\phi(s)=\frac{s^p - p(s-1)-1}{p(p-1)}$ if $p \geq 1$ (the case $p=1$ corresponding to $\D_\phi=\KL$).
%\end{align*}
\vspace*{-0.3cm}
\paragraph{Hellinger-Kantorovich (HK) / Wasserstein-Fisher-Rao distance (WFR).} When $\D_\phi =\KL$, $\C(t) = -\log\cos^2(t\wedge\tfrac{\pi}{2})$ and $q=p=2$, then one has
%\begin{align*}
	$\Dd([u,a], [v,b])^2 = a^2 + b^2 - 2ab\cos(\tfrac{\pi}{2}\wedge |u-v|)$.
%\end{align*}
This construction, which might seem peculiar, corresponds to the one used to make unbalanced OT a geodesic distance, as detailed in~\citep{liero2015optimal,chizat2018unbalanced}. 
\vspace*{-0.3cm}
\paragraph{Partial optimal transport distance (PT).} When $\D_\phi = \TV$, $\C(t)=t^q$, $q\geq 1$ and $p=1$, then
%\begin{align*}
	$\Dd([u,a], [v,b])^q = a + b - (a\wedge b)(2-|u-v|^q)_+$ 
%\end{align*}
defines a cone distance~\citep{chizat2018unbalanced}.
% The setting of HK/WFR might seem peculiar, but it makes unbalanced OT a length space induced by the GH distance when $d$ is a geodesic distance on $X$. PT and HK/WFR introduce cut-offs, i.e. there is no transport between points too far from each other, e.g. in the latter case $\C(d(x,y))=+\infty$ if $d(x,y)>\pi/2$. The cut-off can be modified by scaling $\la \mapsto \la(\cdot/s)$ for some cutoff $s$.

\subsubsection{Definitions and properties}

The conic formulation consists in solving a GW problem on the cone, with the addition of two linear constraints. Informally speaking, $L_c$ from Lemma~\ref{lem-rewrite-ugw} becomes $\Dd$, the term $(|(\mu\otimes\mu)^\bot| + |(\nu\otimes\nu)^\bot|)$ is taken into account by the constraints~\eqref{eq-ugw-conic} below, and the variables $(\f,\g)$ are replaced by $(r^p,s^p)$.
%
It reads  $\CGW(\Xx,\Yy) \eqdef \inf_{\al\in\Uu_p(\mu,\nu)}\Hh(\al)$ where
\begin{equation}\label{eq-ugw-conic}
\begin{aligned}
	 \Hh(\al)\eqdef\int &\Dd([d_X(x,x'), r r'], [d_Y(y,y'), s s'])^q \,\d\al([x,r], [y,s])\d\al([x',r'], [y',s']),
\end{aligned}
\end{equation}
and $\Uu_{p}(\mu,\nu)$ is defined as the set
\begin{equation}
\Uu_{p}(\mu,\nu) \eqdef \left\{
\begin{aligned}
	 \al\in\Mm_+(\Co[X]\times\Co[Y]),\;
	 \int_{\RR_+} r^p \d\al_1(\cdot,r)=\mu,\;
	 \int_{\RR_+} s^p \d\al_2(\cdot,s)=\nu
\end{aligned}
\right\}.
\end{equation}
It is similar to the conic formulation of UW, see Appendix~\ref{sec-app-background}.
%
Note that similarly to the GW formulation~\eqref{eq-defn-gw} -- and in sharp contrast with the conic formulation of UW -- here the transport plans are defined on the cone $\Co[X] \times \Co[Y]$ but the cost $\Dd$ is a distance on $\Co[\RR_+]$.

We present now the main contributions of this paper, proved in Appendix~\ref{appendix-distance-cgw}. We state that CGW defines a distance under conditions that hold for the settings of Section~\ref{sec-setup-dist}, and that it is upper-bounded by $\UGW$. While the distance $\CGW^{1/q}$ 
%
%\redrm{seems difficult to compute} 
%
cannot be casted as a finite dimensional program even in discrete settings (because it is defined on a lifted space), $\UGW$ can be approximated with efficient numerical schemes as detailed in Section~\ref{sec-algo}. The tightness of the bound between $\UGW$ and $\CGW$ and the computation of $\CGW$ are open questions left for future works.
%
\begin{theorem}\label{thm-ugw-dist}
		(i) The divergence $\CGW$ is symmetric, positive and definite up to isometries.
		(ii) If $\Dd$ is a distance on $\Co[\RR_+]$, then $\CGW^{1/q}$ is a distance on the set of mm-spaces up to isometries.
		(iii) For any $(\D_\phi, \C, p, q)$ with associated cost $\Dd$ on the cone, one has $\UGW\geq\CGW$.
\end{theorem}
\paragraph{Sketch of proof}
\textbf{(i)} $\CGW$ is positive and symmetric. Definiteness holds thanks to Proposition~\ref{prop-cone-dist-definite}. \textbf{(ii)} The triangle inequality is similar to balanced OT, and applies the gluing lemma~\citep[Lemma 7.6]{villani2003}. The non-trivial part is showing that the latter lemma holds, because it glues two plans provided they have a common marginal. Since $\CGW$ is invariant under radial rescalings (called dilations in Appendix~\ref{appendix-distance-cgw}), it is possible to dilate two plans such that they have a common marginal and remain optimal.
%
\textbf{(iii)} Take an optimal plan $\pi$ for $\UGW(\Xx,\Yy)$. From this $\pi$ one can build a plan $\al$ such that $\Ll(\pi)\geq \Hh(\al)$ because $L_c\geq H_c$. Furthermore $\al\in\Uu_p$, and is thus admissible and suboptimal, which yields $\UGW(\Xx,\Yy)=\Ll(\pi)\geq\Hh(\al)\geq\CGW(\Xx,\Yy)$.


%\subsubsection{Preliminary results}
%
%We present concepts and properties which are necessary for the proofs of Theorem~\ref{thm-ugw-dist} and Theorem~\ref{thm-ineq-formul}.
%
%\begin{definition}[dilations]
%	Consider $v([x, r], [y, s])$ a Borel measurable scaling function depending on $[x, r], [y, s]\in\Co[X]\times\Co[Y]$. Take a plan $\al\in\Mm_+(\Co[X]\times\Co[Y])$. We define the dilation $\dil{v}: \al\mapsto (h_v)_\sharp(v^{p}\al)$ where
%		$h_v([x, r], [y, s]) \eqdef ([x, r/w], [y, s/w])$,
%	and $w = v([x, r], [y, s])$. It reads for any test function $\xi$
%	\begin{align*}
%		\int \xi([x, r], [y, s])\d\dil{v}(\al) = \int\xi([x, r/w], [y, s/w])w^p \d\al.
%	\end{align*}
%\end{definition}
%A crucial property of the conic formulation~\eqref{eq-ugw-conic} is its invariance to dilations of the radial coordinates.
%%
%We state this invariance in the following lemma. The proof can be found in Appendix~\ref{appendix-distance-cgw}.
%\begin{lemma}[Invariance to dilation]
%	The problem $\CGW$ is invariant to dilations, i.e. for any $\al\in\Uu_p(\mu,\nu)$, we have $\dil{v}(\al)\in\Uu_p(\mu,\nu)$ and $\Hh(\al) = \Hh(\dil{v}(\al))$.
%\end{lemma}
%The invariance to dilation allows one to normalize the plan $\al$ and assume extra properties without loss of generality.
%%
%For instance with $v=\al(\Co[X]\times\Co[Y])^{-1/q}$ we can assume that $\al$ is a probability distribution, which allows us to leverage results of balanced optimal transport on the cone. It can also be leveraged to prove the following lemma, which is used to prove the triangle inequality.
%
%\begin{lemma}[Normalization lemma]\label{lem-norm}
%	Assume there exists $\al\in\Uu_p(\mu,\nu)$ s.t. $\CGW(\Xx,\Yy)=\Hh(\al)$. Then there exists $\tilde{\al}$ such that $\tilde{\al}\in\Uu_p(\mu,\nu)$, $\CGW(\Xx,\Yy)=\Hh(\tilde{\al})$ and whose marginal on $\Co[Y]$ is
%	$\nu_{\Co[Y]}= \delta_{\zc_Y} + \margc_\sharp(\nu \otimes \delta_1)$,
%	where $\margc :X\times\RR_+ \rightarrow\Co[X]$ is the canonical injection into the cone that reads $\margc(x,r)\eqdef[x,r]$.
%\end{lemma}


==> sections/checklist-neurips.tex <==
\newpage
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Due to the scalability of the method, it might have a limited immediate impact with respect to individual and societal aspects.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix~\ref{appendix-distance-ugw} and~\ref{appendix-algo}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{sec-xp} and Appendix~\ref{sec-app-xp}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See standard deviation table in Appendix~\ref{sec-app-xp}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{sec-app-xp}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{Datasets are open source.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See the supplementary material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{The datasets used involve no individual data.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{The datasets used involve no individual data.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
   \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

\newpage
